IsoGeometric Suitable Coupling Methods for Partitioned Multiphysics Simulation with Application to Fluid-Structure Interaction

This paper presents spline-based coupling methods for partitioned multiphysics simulations, specifically designed for isogeometric analysis (IGA) based solvers. Traditional vertex-based coupling approaches face significant challenges when applied to IGA solvers, including geometric accuracy issues, interpolation errors, and substantial communication overhead. The methodology draws on the IGA mathematical framework to deliver coupling solutions that preserve high-order continuity and exact geometric representation of splines. We develop two complementary strategies: (1) a spline-vertex coupling method enabling efficient interaction between IGA and conventional solvers, and (2) a fully isogeometric coupling approach maximizing accuracy for IGA-to-IGA communication. Both theoretical analysis and extensive numerical experiments demonstrate that our spline-based methods significantly reduce communication overhead compared to traditional approaches while enhancing geometric accuracy through exact boundary representation and maintaining higher-order solution continuity across coupled interfaces. We quantitatively confirm communication efficiency benefits through systematic measurements of transfer times and data volumes across various mesh refinement levels. Our benchmark studies demonstrate geometric fidelity advantages while highlighting how splines naturally preserve solution derivatives across interfaces without requiring additional computation. This work provides efficient coupling strategies tailored to IGA-based solvers and establishes a practical bridge between IGA and traditional discretization methods, enabling broader adoption of IGA in established simulation workflows.

==> figures/data_experimental_spline_combined.tex <==
% \documentclass[tikz]{standalone}
% \usepackage{pgfplots}
% \pgfplotsset{compat=newest}
% \usepackage{amsmath}
% \usepackage{xcolor}

% \begin{document}


% \caption{Comparison of measured and estimated communication overhead in IGA with varying polynomial degree $p$.}
% \end{document}

==> figures/experimental_quad_spline.tex <==
% \documentclass{standalone}
% \usepackage{pgfplots}
% \pgfplotsset{compat=newest}
% \usepackage{amsmath}
% \usepgfplotslibrary{colorbrewer}

% 定义红蓝不同深浅的循环色表
% \pgfplotscreateplotcyclelist{customcolorlist}{
%     {red!40!white, solid, dashed},     % Theory p=3
%     {blue!40!white, mark=*},   % Exp p=3
%     {red!70!white, solid, dashed}, % Theory p=4
%     {blue!70!white, mark=*}, % Exp p=4
%     {red, solid, dashed},     % Theory p=5
%     {blue, mark=*}    % Exp p=5
% }
% 
% \begin{document}
% \begin{tikzpicture}[baseline]
% \begin{axis}[
%     width=\linewidth,
%     height=9cm,
%     xmode=log,
%     log basis x=2,
%     % ymode=log,
%     xlabel={Number of parameter subdivisions per direction \(r\)},
%     ylabel={Total communication size (KB)},
%     % title={Communication Overhead: Quadrature v.s Splines $(N_t=1)$},
%     grid=both,
%     grid style={dashed, gray!30},
%     legend style={at={(0.02,0.98)},anchor=north west},
%     every axis plot/.append style={line width=1pt},
%     cycle list name=customcolorlist,
%     mark options={solid},
%     xtick={2,4,8,16,32,64,128},
%     xticklabels={2,4,8,16,32,64,128}
% ]

% % ---------- p=3 ----------
% \addplot coordinates {(2,1.5)(4,6)(8,24)(16,96)(32,384)(64,1536)(128,6144)};
% \addlegendentry{\(O_{\text{quad}},\; p=3\)}

% \addplot coordinates {(2, 0.867188) (4, 1.49219) (8, 3.30469) (16, 9.17969) (32, 29.9297) (64, 107.43) (128, 406.43)};
% \addlegendentry{\(O_{\text{spline}},\; p=3\)}

% % ---------- p=4 ----------
% \addplot coordinates {(2,2.34375)(4,9.375)(8,37.5)(16,150)(32,600)(64,2400)(128,9600)};
% \addlegendentry{\(O_{\text{quad}},\; p=4\)}

% \addplot coordinates {(2, 1.1875) (4, 1.90625) (8, 3.90625) (16, 10.1562) (32, 31.6562) (64, 110.656) (128, 412.656)};
% \addlegendentry{\(O_{\text{spline}},\; p=4\)}

% % ---------- p=5 ----------
% \addplot coordinates {(2,3.375)(4,13.5)(8,54)(16,216)(32,864)(64,3456)(128,13824)};
% \addlegendentry{\(O_{\text{quad}},\; p=5\)}

% \addplot coordinates {(2, 1.55469) (4, 2.36719) (8, 4.55469) (16, 11.1797) (32, 33.4297) (64, 113.93) (128, 418.93)};
% \addlegendentry{\(O_{\text{spline}},\; p=5\)}

% \end{axis}
% \end{tikzpicture}


==> figures/perpendicular-flap-tip-displacement.tex <==
% \documentclass[tikz]{standalone}
% \usepackage{pgfplots}
% \pgfplotsset{compat=1.18}
% \usepgfplotslibrary{colormaps}

% \begin{document}
% \begin{tikzpicture}
%   \begin{axis}[
%     width=13cm, height=8cm,
%     xlabel={Time (s)},
%     ylabel={Tip displacement in \(x\) (m)},
%     font=\small,  % ← 使用默认 serif 字体
%     grid=major,
%     major grid style={gray!20, densely dotted},
%     legend style={
%       at={(0.5,-0.2)},
%       anchor=north,
%       font=\small,
%       draw=none,
%       fill=none,
%       legend columns=3,
%     },
%     cycle list={
%       {gray!60!green, thick, solid},            % calculix
%       {gray!30!red, thick, dashed},             % dealii
%       {gray!50!teal, thick, dotted},            % dune
%       {gray!30!orange, thick, dash dot},        % fenics
%       {gray!30!purple, thick, densely dotted},  % nutils
%       {blue!70!gray, very thick, solid},        % gismo (highlight)
%     },
%     clip=true
%   ]

%     \addplot+[] table[col sep=space, header=true, x=Time, y=Displacement0]
%       {doc/openfoam-calculix-v2404.log};
%     \addlegendentry{CalculiX}

%     \addplot+[] table[col sep=space, header=true, x=Time, y=Displacement0]
%       {doc/openfoam-dealii-v2404.log};
%     \addlegendentry{deal.II}

%     \addplot+[] table[col sep=space, header=true, x=Time, y=Displacement0]
%       {doc/openfoam-dune-v2404.log};
%     \addlegendentry{DUNE}

%     \addplot+[] table[col sep=space, header=true, x=Time, y=Displacement0]
%       {doc/openfoam-fenics-v2404.log};
%     \addlegendentry{FEniCS}

%     \addplot+[] table[col sep=space, header=true, x=Time, y=Displacement0]
%       {doc/openfoam-nutils-v2404.log};
%     \addlegendentry{Nutils}

%     \addplot+[] table[col sep=space, header=true, x=Time, y=Displacement0]
%       {doc/openfoam-gismo-v2404.log};
%     \addlegendentry{\textbf{G+Smo}}

%   \end{axis}
% \end{tikzpicture}
% \end{document}

==> figures/timing_solidread.tex <==
% \documentclass[tikz]{standalone}
% \usepackage[margin=1in]{geometry}
% \usepackage{textcomp}
% \usepackage{pgfplots}
% \pgfplotsset{width=0.8\textwidth}
% \begin{document}
% \begin{tikzpicture}[baseline]
% \begin{axis}[
%     ybar,                           % 柱状图样式
%     bar width=8pt,                  % 柱子的宽度
%     enlargelimits=0.15,
%     symbolic x coords={2,4,8,16,32,64,128}, % 离散的横坐标
%     xtick=data,
%     ylabel={Dimensionless Communication Time},
%     xlabel={Number of parameter subdivisions $r$ per direction (for $r\in\{1,2,...,7\}$)},
%     legend style={at={(0.03,0.97)}, anchor=north west, font=\small},
%     grid=both,
%     width=14cm,
%     height=9cm,
%     thick,
%     tick style={black},
%     every axis plot/.append style={line width=1pt},
%     % title={Experimental Communication Overhead ($N_t=10000$)},
% ]
% % Spline p=3
% \addplot+[fill=red!50, draw=red, bar shift=-15pt] coordinates {
%     (2, 1.0)
%     (4, 0.7919565911267156)
%     (8, 0.8887328439195659)
%     (16, 0.9484200446856048)
%     (32, 0.9386530481966167)
%     (64, 1.0570060644749442)
%     (128, 1.1573571656559207)
% };
% % Spline p=4
% \addplot+[fill=red!70, draw=red, bar shift=-9pt] coordinates {
%     (2, 1.0)
%     (4, 0.7803901304740989)
%     (8, 0.9711277612711536)
%     (16, 0.9901175558713344)
%     (32, 0.9358609998708176)
%     (64, 1.0704689316625757)
%     (128, 1.1676785944968349)
% };
% % Spline p=5
% \addplot+[fill=red!90, draw=red, bar shift=-3pt] coordinates {
%     (2, 1.0)
%     (4, 1.0378112102250034)
%     (8, 1.013114099320996)
%     (16, 1.018506190919984)
%     (32, 1.0238982825189722)
%     (64, 1.1111702835840769)
%     (128, 1.211489814938091)
% };
% % Quadrature p=3
% \addplot+[fill=blue!50, draw=blue, bar shift=3pt] coordinates {
%     (2, 1.0)
%     (4, 1.3416068982190343)
%     (8, 2.411556128616327)
%     (16, 4.465790958175518)
%     (32, 8.561044403255702)
%     (64, 18.41614956886131)
%     (128, 34.94415343702151)
% };
% % Quadrature p=4
% \addplot+[fill=blue!70, draw=blue, bar shift=9pt] coordinates {
%     (2, 1.0)
%     (4, 1.5494239377706025)
%     (8, 2.6280179056285315)
%     (16, 4.916782857562192)
%     (32, 10.006971453731563)
%     (64, 20.299772510457178)
%     (128, 34.91326043883466)
% };
% % Quadrature p=5
% \addplot+[fill=blue!90, draw=blue, bar shift=15pt] coordinates {
%     (2, 1.0)
%     (4, 1.478777292576)
%     (8, 2.877554585152838)
%     (16, 5.45703056768559)
%     (32, 11.766026200873362)
%     (64, 28.49371179039301)
%     (128, 56.55013100436681)
% };

% \legend{Spline $p=3$, Spline $p=4$, Spline $p=5$, Quadrature $p=3$, Quadrature $p=4$, Quadrature $p=5$}
% \end{axis}
% \end{tikzpicture}
% \end{document}

==> nonlinear_plot.tex <==
\begin{tikzpicture}[baseline]
\begin{groupplot}[
    group style={
        group name=myplot,
        group size=1 by 2,
        vertical sep=20pt,
        xticklabels at=edge bottom
    },
    width=13cm,
    height=5.5cm,
    grid=major,
    xlabel style={font=\small},
    ylabel style={font=\small},
    ticklabel style={font=\footnotesize},
    legend style={
        at={(0.5,-1.5)},
        anchor=north,
        legend columns=3,
        font=\footnotesize,
        draw=none,
        fill=none,
        /tikz/every even column/.append style={column sep=0.5cm}
    },
    legend cell align=left
]

% Upper plot: uy
\nextgroupplot[ylabel={Displacement $u_y\;[\mathrm{m}]$}]
\addplot+[mark=square*, mark options={fill=gray}, smooth, mark repeat=5, line width=1pt] 
    table[x index=3, y index=1, col sep=comma] {Data/NonlinearLoad/pointData-vertex-vertex.csv};
\addlegendentry{Vertex-Vertex}

\addplot+[mark=o, mark options={fill=blue}, smooth, mark repeat=5, line width=1pt] 
    table[x index=3, y index=1, col sep=comma] {Data/NonlinearLoad/pointData-IGA-vertex.csv};
\addlegendentry{Spline-Vertex}

\addplot+[mark=triangle*, mark options={fill=red}, smooth, mark repeat=5, line width=1pt] 
    table[x index=3, y index=1, col sep=comma] {Data/NonlinearLoad/pointData-IGA-IGA.csv};
\addlegendentry{Spline-Spline}

% Lower plot: uz
\nextgroupplot[xlabel={$t\;[\mathrm{s}]$}, ylabel={Displacement $u_z\;[\mathrm{m}]$}]
\addplot+[mark=square*, mark options={fill=gray}, smooth, mark repeat=5, line width=1pt] 
    table[x index=3, y index=2, col sep=comma] {Data/NonlinearLoad/pointData-vertex-vertex.csv};

\addplot+[mark=o, mark options={fill=blue}, smooth, mark repeat=5, line width=1pt] 
    table[x index=3, y index=2, col sep=comma] {Data/NonlinearLoad/pointData-IGA-vertex.csv};

\addplot+[mark=triangle*, mark options={fill=red}, smooth, mark repeat=5, line width=1pt] 
    table[x index=3, y index=2, col sep=comma] {Data/NonlinearLoad/pointData-IGA-IGA.csv};

\end{groupplot}
\end{tikzpicture}


==> turek-hron-fsi3.tex <==
\begin{tikzpicture}
\begin{axis}[
    width=12cm,
    height=8cm,
    grid=both,
    xlabel={time [s]},
    ylabel={y-displacement [m]},
    title={y-displacement of the flap tip},
    xmin=5, xmax=6.5,
    legend style={at={(0.5,-0.2)}, anchor=north, legend columns=1},
    legend cell align={left}
]

\addplot[
    color=green,
    thick,
    solid
] table [x index=0, y index=4, col sep=space] {validation_data/precice-Solid-watchpoint-Flap-Tip-r3-run.log};
\addlegendentry{Gismo Solid (r 3, degree 2)}

\addplot[
    color=blue,
    thick,
    dashed
] table [x index=0, y index=4, col sep=space] {validation_data/precice-Solid-watchpoint-Flap-Tip-r4-run.log};
\addlegendentry{Gismo Solid (r 4, degree 2)}

\addplot[
    color=red,
    thick,
    dotted
] table [x index=0, y index=11, col sep=space] {validation_data/ref_fsi3.point};
\addlegendentry{Reference Data}

\end{axis}
\end{tikzpicture}


